Gradient Einstein-type warped products: rigidity, existence and nonexistence results via a nonlinear PDE

We establish the necessary and sufficient conditions for constructing gradient Einstein-type warped metrics. One of these conditions leads us to a general Lichnerowicz equation with analytic and geometric coefficients for this class of metrics on the space of warping functions. In this way, we prove gradient estimates for positive solutions of a nonlinear elliptic differential equation on a complete Riemannian manifold with associated Bakry-\'Emery Ricci tensor bounded from below. As an application, we provide nonexistence and rigidity results for a large class of gradient Einstein-type warped metrics. Furthermore, we show how to construct gradient Einstein-type warped metrics, and then we give explicit examples which are not only meaningful in their own right, but also help to justify our results.

==> pre/auth.tex <==
\title{Einstein-type manifolds}
\author{
  Author A
\and
Author B
 % \and
 % Elismar Batista
}
%Nonexistence results for warped product gradient Einstein-type manifolds
% \ead{willian.tokura@ufac.br}
% \ead{bezerra@ufg.br}
% \ead{elismardb@gmail.com}

% \address[1]{\textup{Universidade Federal do Acre, CCET, 69920--900, Rio Branco---AC, Brazil}}
% \address[2]{\textup{Universidade Federal de Goi\'{a}s, IME, 131, 74001--970, Goi\^{a}nia---GO, Brazil}}
% \address[3]{\textup{Instituto Federal do Tocantins, IFTO, 77300--000, Tocantins---TO, Brazil}}

% \fntext[orcid1]{https://orcid.org/0000--0001--9363--793X}
% \fntext[orcid2]{https://orcid.org/0000--0003--4258--4676}
% \fntext[orcid3]{https://orcid.org/0000--0002--4391--4238}

% \begin{keyword}
%   Einstein-type manifolds, warped product manifolds, Li-Yau gradient estimates.
%   \MSC[2010]53C21\sep{53C24}\sep{53C25}\sep{53C44}
% \end{keyword}


==> pre/thms.tex <==
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{question}[theorem]{Question}

